Learning Strategies For Successful Crowd Navigation

Teaching autonomous mobile robots to successfully navigate human crowds is a challenging task. Not only does it require planning, but it requires maintaining social norms which may differ from one context to another. Here we focus on crowd navigation, using a neural network to learn specific strategies in-situ with a robot. This allows us to take into account human behavior and reactions toward a real robot as well as learn strategies that are specific to various scenarios in that context. A CNN takes a top-down image of the scene as input and outputs the next action for the robot to take in terms of speed and angle. Here we present the method, experimental results, and quantitatively evaluate our approach.

==> _2_Background/main.tex <==
\section{Background}
REMOVE THIS SECTION - RELATED WORK IS IN THE INTRO
%\begin{itemize}
%\item Previous work done on many model-based approaches - social psych/cog sci (Luber, 2012 - not in real world, not sure if they scale).  Similar to Luber, 2012, we also believe pro-social behaviors are better learned from real-world experiments rather than modelled.
%\item While learning from publicly available surveillance data sets is an improvement over modelling one drawback is the behavior being learned is for a human navigating amongst humans. It does not take into account the behavior of humans around an actual robot as we do in our experiments. In addition, humans may use various strategies, gentle pressure/touch, tapping on the shoulder, natural language and hand and arm gestures (reference smithsonian 2012 article) that may not be possible or as effective for a robot.  Furthermore it is questionable whether these strategies are detectable in the coarse-grain afforded by surveillance video.
%\item Evaluation criteria - human rules of the road/socially aware (Luber, 2012)
%\begin{itemize}
%\item Social awareness - comfort
%\item More quantitative criteria - Travel time, path length 
%\end{itemize}
%
%\item Machine Learning approach - Le Fan Chen, MIT (2018)
%\item Recently there has been surge of using deep learning for Robot navigation, one such example is \cite{long2017deep} where deep learning is used for multi-agent navigation with goal of collision avoidance. In this particular paper, the end-to-end framework is implemented as Deep Neural Networks (DNNs). To train the network, extensive dataset was collected consisting of frames showing how an agent should avoid its surrounding agents. Each frame includes both the agent’s observation about other agents and the agent’s reactive collision avoidance strategy in terms of the steering velocity. Although in our experiment we use single agent crowd navigation but the concept of using neural network for learning the crowd behaviour is similar. 
%\item \cite{aroor2018online} formulates a Bayesian approach that relies only on an onboard range scanner to learn a global crowd model online. Although it doesn’t use neural network for learning but it does learn about the crowd behaviour with help of sensors and algorithms designed to learn the global crowd behaviour which agent follows. 
%\item In \cite{zhao2008segmentation} research approach, each robot uses online machine learning techniques to adapt dynamically its behavior to the local conditions. Similar to this we use deep neural network to learn the crowd behaviour.
%\end{itemize}
